Selective Self-Assembly using Re-Programmable Magnetic Pixels

This paper introduces a method to generate highly selective encodings that can be magnetically "programmed" onto physical modules to enable them to self-assemble in chosen configurations. We generate these encodings based on Hadamard matrices, and show how to design the faces of modules to be maximally attractive to their intended mate, while remaining maximally agnostic to other faces. We derive guarantees on these bounds, and verify their attraction and agnosticism experimentally. Using cubic modules whose faces have been covered in soft magnetic material, we show how inexpensive, passive modules with planar faces can be used to selectively self-assemble into target shapes without geometric guides. We show that these modules can be easily re-programmed for new target shapes using a CNC-based magnetic plotter, and demonstrate self-assembly of 8 cubes in a water tank.

==> 0-abstract.tex <==

\begin{abstract}

This paper introduces a method to magnetically "program" physical components to assemble in chosen configurations. We leverage Hadamard matrices to introduce a theoretical basis for how to design the faces of components to be maximally attractive to their intended mate, while remaining maximally agnostic to other faces, and derive guarantees on these bounds. We use passive, soft magnetic material on the faces of components as the basis for actuation, and build a magnetic plotter to program these with the desired signatures. Finally, we demonstrate the merit of this framework with applications that include self-assembly, XXX and XXX.

\end{abstract}



%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% http://dl.acm.org/ccs.cfm

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121.10003124.10010866</concept_id>
<concept_desc>Human-centered computing~Human-computer interaction</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Human-computer interaction}
% \ccsdesc[500]{Human-centered computing~Haptic devices}

\keywords{self-assembly; swarm user interfaces; interactive devices; fabrication}



==> IROS 22 - Stochastic Self-Assembly/0-abstract.tex <==

\begin{abstract}

This paper introduces a method to magnetically "program" physical components to assemble in chosen configurations. We leverage Hadamard matrices to introduce a theoretical basis for how to design the faces of components to be maximally attractive to their intended mate, while remaining maximally agnostic to other faces, and derive guarantees on these bounds. We use passive, soft magnetic material on the faces of components as the basis for actuation, and build a magnetic plotter to program these with the desired signatures. Finally, we demonstrate the merit of this framework with applications that include self-assembly, XXX and XXX.

\end{abstract}



%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% http://dl.acm.org/ccs.cfm

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121.10003124.10010866</concept_id>
<concept_desc>Human-centered computing~Human-computer interaction</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Human-computer interaction}
% \ccsdesc[500]{Human-centered computing~Haptic devices}

\keywords{self-assembly; swarm user interfaces; interactive devices; fabrication}


